Interplay of quantum confinement and strain effects in type I to type II transition in Ge/Si core-shell nanocrystals

The electronic properties of hydrogenated, spherical, Si/Ge and Ge/Si core-shell nanocrystals with a diameter ranging from 1.8 to 4.0 nm are studied within Density Functional Theory. Effects induced by quantum confinement and strain on the near-band-edge states localization, as well as the band-offset properties between Si and Ge regions, are investigated in detail. On the one hand, we prove that Si(core)/Ge(shell) nanocrystals always show a type II band-offset alignment, with the HOMO mainly localized on the Ge shell region and the LUMO mainly localized on the Si core region. On the other hand, our results point out that a type II offset cannot be observed in small (diameter less than 3 nm) Ge(core)/Si(shell) nanocrystals. In these systems, quantum confinement and strain drive the near-band-edge states to be mainly localized on Ge atoms inducing a type I alignment. In larger Ge(core)/Si(shell) nanocrystals, instead, the formation of a type II offset can be engineered by playing with both core and shell thickness. The conditions that favor the transition from a type I to a type II alignment for Ge(core)/Si(shell) nanocrystals are discussed in detail.

==> Table_1.tex <==
\begin{table*}[h!]
\centering
\caption{DFT-LDA energy gaps calculated for Ge(core)/Si(shell) and Si(core)/Ge(shell) of different compositions and size are reported in the table. As a reference, for the smaller NCs, the pristine Ge$_{147}$H$_{100}$ and Si$_{147}$H$_{100}$ show an energy gap of 2.25 and 2.19 eV, respectively. For what concerns the Ge$_{35}$Si$_{122}$H$_{100}$, we have also calculated the  GW energy gap which settles to 3.5 eV.}
\label{SiGe_gaps}
\begin{tabular}{c c c c c}
 \hline
  \multicolumn{1}{|c|}{\bf diameter (nm)} &  
 \multicolumn{1}{|c|}{\bf Ge(core)/Si(shell)} &  
\multicolumn{1}{|c|}{\bf Energy Gap (eV)} & 
\multicolumn{1}{|c|}{\bf Si(core)/Ge(shell)} &  
\multicolumn{1}{|c|}{\bf Energy Gap (eV)}  \\
 \hline
 1.8 & Ge$_{17}$Si$_{130}$H$_{100}$ &  2.09 &  Si$_{17}$Ge$_{130}$H$_{100}$ & 2.10 \\
 1.8 &  Ge$_{35}$Si$_{122}$H$_{100}$ & 2.12 &   Si$_{35}$Ge$_{122}$H$_{100}$ & 2.12 \\
 1.8 &   Ge$_{47}$Si$_{100}$H$_{100}$ & 2.11 &   Si$_{47}$Ge$_{100}$H$_{100}$ & 2.12 \\
 1.8 &   Ge$_{71}$Si$_{76}$H$_{100}$ & 2.16 &   Si$_{71}$Ge$_{76}$H$_{100}$ &  2.10 \\
 \hline
 2.4 & Ge$_{71}$Si$_{222}$H$_{1772}$ &  1.54 &  Si$_{71}$Ge$_{222}$H$_{172}$ & 1.67 \\
 \hline
 3.0 & Ge$_{147}$Si$_{486}$H$_{300}$ &  1.19 &  Si$_{147}$Ge$_{486}$H$_{300}$ & 1.19 \\
 3.0 & Ge$_{71}$Si$_{562}$H$_{300}$ &  1.17 &  -   & - \\
 \hline
 4.0 & Ge$_{220}$Si$_{1192}$H$_{510}$ &  0.83 &  -   & -  \\
 \hline
\end{tabular}
\end{table*}


